Improving Fairness and Mitigating MADness in Generative Models

Generative models unfairly penalize data belonging to minority classes, suffer from model autophagy disorder (MADness), and learn biased estimates of the underlying distribution parameters. Our theoretical and empirical results show that training generative models with intentionally designed hypernetworks leads to models that 1) are more fair when generating datapoints belonging to minority classes 2) are more stable in a self-consumed (i.e., MAD) setting, and 3) learn parameters that are less statistically biased. To further mitigate unfairness, MADness, and bias, we introduce a regularization term that penalizes discrepancies between a generative model's estimated weights when trained on real data versus its own synthetic data. To facilitate training existing deep generative models within our framework, we offer a scalable implementation of hypernetworks that automatically generates a hypernetwork architecture for any given generative model.

==> Sections/more_details_ple.tex <==
\subsection{More Details on PLE}
\label{sec:more_details_ple}
Consider a matrix of random variables $\mX$, which are independent and identically distributed (I.I.D.) outcomes from a distribution with true parameters $\theta$.  We write $\mX = [\vx_1, \dots \vx_n], \vx_i \sim P(\theta), i = 1, \dots, n$.  We use $\mX$ to form an estimate $\hat{\theta}$ of the true parameters $\theta,$ which are unknown.  Because $\theta$ is fixed, $\hat{\theta}$ is random due to the uncertainty in estimation, and we can thus write the probability density function (PDF) of $\hat{\theta}$ in terms of the density of $\mX$.  With the PDF of a single outcome $\vx$ described by $f_{\vx; \theta}(\va) = P(\vx = \va; \theta)$, we can write the probability distribution of $\mX$ as follows, noting that $\mA = [\va_1, \dots, \va_n]$:
\begin{equation*}
    f_{\mX}(\mA; \theta) = P(\vx_1 = \va, \vx_2 = \va, \dots, \vx_n = \va; \theta)
\end{equation*}
Because the data are assumed to be independent, we can simplify this to 
\begin{equation*}
    f_{\mX}(\mA; \theta) = \prod_{i=1}^n P(\vx_i = \va_i; \theta)
\end{equation*}
And incorporating the assumption that each $\vx_i$ are identical, we can remove this product's dependence on $i$ to get
\begin{equation}
\label{eq:joint_prod}
    f_{\mX}(\mA; \theta) = \prod_{i=1}^n P(\vx = \va_i; \theta).
\end{equation}
Our goal is to get a PDF of our estimate, $\hat{\theta}$.  We start by creating an estimate $\hat{\theta}_i$ from a single data point $\vx_i,$ and we introduce a function $h$ which which (deterministically) chooses  $\hat{\theta}_i$ from $\vx_i$.  In this case, $h$ is an ``estimation function'' which creates an estimate from the data.  We do this so we can directly relate the PDF of $\vx_i$ to the PDF of $\hat{\theta_i}$:

\[\hat{\theta_i} = h(\vx_i) \implies f_{\hat{\theta_i}}(\vb_i) = P(h(\vx_i) = \vb_i), \]
If $h$ is invertible, we can write the PDF of $\hat{\theta_i}$ in terms of the PDF of $\vx_i,$ as $h^{-1}$ explicitly relates $\hat{\theta_i}$'s PDF to $\vx_i$'s.  This is useful because we already assumed $\vx_i$ has an explicit parametric form, and the parameters we estimate from the data should intuitively be related to the true parameters underlying the data's true distribution.
\[f_{\hat{\theta_i}}(\vb_i) = P(\vx_i = h^{-1}(\vb_i)).\]

The above expression gives us a local estimate of our parameters $\hat{\theta_i}$ from each individual datapoint $\vx_i$, however our goal is a global estimate for the entire dataset $\mX$ consisting of $n$ datapoints.  As a result, we can use the local estimate from each datapoint, $\vb_i,$ to create a global estimate $\hat{\vb}$ as follows:
\begin{equation}
    \label{eq:define_big_h}
    \hat{\vb} = H(\mX) = \frac{1}{n} \sum_{i=1}^n \vb_i = \frac{1}{n} \sum_{i=1}^n h(\vx_i)
\end{equation}
To justify this choice of our global estimate, first note that each $\vx_i \in \mX$ are assumed to be identical and independent.  As a result, each local estimate's contribution to the global estimate should be invariant to permutations of the data, accounting for the $\frac{1}{n}$ present in the summation.  Furthermore, because the data is random, our global estimate $H(\mX)$ will be random as well, with its probability being related to both $\mX$ and the number of possible ``ways'' one can estimate the same parameter from different datasets.  

Our goal now is to write the PDF of our global estimate $\hat{\theta}$ in terms of the PDF of our data $\mX$. 
We begin by writing the PDF of our global estimate as follows:

% We can now write the PDF of $\hat{\theta}$ in terms of $\mA$ and $\mX$
% \[f_{\hat{\theta}}(\mA; \theta) = \prod_{i=1}^n P(\vx = h^{-1}(\va_i); \theta) \]

% How can we encorce all of each of these are the same?  $h(x_i) = a \; \forall i$ 
% Just define $H$ this way and justify why - we want 
% Use $b$ above instead of $a$ when $h$ is not preset
% Why $H$
% \begin{itemize}
%     \item Needs to be permutation independent (because they are independent)
%     \item Each needs to contribute equally (because they are identical) 
% \end{itemize}
% With these results, we can now turn to the PDF of an estimate $\hat{\theta}$ from a random matrix $\mX.$  Since each random vector $\vx_i \in \mX$ has the same distribution, we can write out the PDF as a function of estimates from each individual $\vx_i.$  The important observation is that all of these datapoints are assumed to come from the same distribution, and there are many ways that the data could have been generated from a model with the same parameters.  We can make this assumption explicit by assuiming each $\va \in \mA$ are related, and that each $\vx \in \mX$ was drawn from the same distribution - one parametrized by $\hat{\theta}$

% Consider an estimator $H(\mX)$ from a set of $n$ independent and identically distributed (I.I.D.) samples from a distribution $D(\theta),$ where $mX = [\vx_1, \dots \vx_n], \vx_i \sim D(\theta), i = 1, \dots, n$  Assuming $H$ is deterministic\footnote{This means there is no randomness introduced by $H$; all the ``randomness'' or uncertainty in estimating $H$ comes from the data itself.}, we can write the probability density function of $\hat{\theta}$ in terms of the data: $f_{\hat{\theta}}(a) =  P(H(\mX) = a).$  

% First, consider the case when $n=1$.  

% Now, when $n > 1$, we write $H(\mX)$ in terms of the joint PDF, which is separable because the data are assumed to be I.I.D..  Furthermore, the I.I.D. assumption tells us that the order of the data does not matter, and we can build up an estimate of our parameters by combining the individual estimates from each data point, noting that each individual estimate should factor in equally to our overall estimate of $\hat{\theta}.$  
% Let $\hat{\va} = H(\mX) = \frac{1}{n} \sum_{i=1}^n h(\vx_i),$ and consider the PDF of $\hat{\theta}$
\[f_{\hat{\theta}}(\hat{\vb}) = P(H(\mX) = \hat{\vb}) = P\left(\frac{1}{n} \sum_{i=1}^n h(\vx_i) = \hat{\vb} \right) \]
We can write this PDF in terms of each $\vx_i$ as follows:
\[
f_{\hat{\theta}} (\hat{\vb}) = \int_{\vb_1}\dots \int_{\vb_n} P\left(h(\vx_1) = \vb_1, \dots, h(\vx_n) = \vb_n\right) d\vb_1, \dots d\vb_n  \; \text{s.t.} \; \frac{1}{n} \sum_{i=1}^n \vb_i = \hat{\vb}
\]
\lolo{Are we actually integrating here? Because this is a PDF, we are just evaluating it. In fact this integral is effectively "destroyed" via deltas places at $\alpha_i$}
Incorporating our independence assumption again, we have:
\[
f_{\hat{\theta}} (\hat{\vb}) = \int_{\vb_1}\dots \int_{\vb_n} \prod_{i=1}^n P(\vx = h^{-1}(\vb_i)) d\vb_1, \dots d\vb_n \; \text{s.t.} \; \frac{1}{n} \sum_{i=1}^n \vb_i = \hat{\vb}.
\]
Consider the case when $n=2$ first:
\[f_{\hat{\theta}} (\hat{\vb}) = \int_{\vb_1} \int_{\vb_2} P(\vx = h^{-1}(\vb_1)) \cdot P(\vx = h^{-1}(\vb_2)) d\vb_1 d\vb_2 \; \text{s.t.} \; \vb_1 + \vb_2 = 2\hat{\vb}\]
This can be simplified to a single integral, which is clearly a convolution of the PDF with itself:
\[
f_{\hat{\theta}} (\hat{\vb}) = \int_{\vs} P(\vx = h^{-1}(\vs)) \cdot P(\vx = h^{-1}(2\vb - \vs)) d\vs = (f_{\vx} \ast f_{\vx}) (h^{-1}(2\vs))
\]
\lolo{I do not see anything wrong with the convolution part, but I don't understand why you use the $h^{-1}$ formulation. Do you even need it?}
In general, for $n$ I.I.D. datapoints, we have 
\begin{multline*}
    f_{\hat{\theta}}(\hat{\vb}) = \int_{\vs_1} \int_{\vs_2} \dots \int_{\vs_{n-1}} (f_{\vx} \circ h) (\vs_1) \cdot (f_{\vx} \circ h)(\vs_2 - \vs_1) \cdot \hdots \\ \cdot (f_{\vx} \circ h) \left(n \cdot \hat{\vb} - \sum_{i=1}^{n-1}s_i\right) d\vs_1, \dots d\vs_{n-1}
\end{multline*}

\begin{multline}
    f_{\hat{\theta}}(\hat{\vb}) = \int_{\vs_1} \int_{\vs_2} \dots \int_{\vs_{n-1}} \prod_{i=1}^{n-1} (f_{\vx} \circ h) \left(\vs_i - \sum_{j=1}^{i-1} \vs_j \right) \cdot \\(f_{\vx} \circ h) \left( n \cdot \hat{\vb} - \sum_{i=1}^{n-1} \vs_i \right) d\vs_1 \cdot \dots \cdot d\vs_{n-1}
\end{multline}

\begin{align}
\implies f_{\hat{\theta}} (\hat{\vb}) &= (\underbrace{f_{\vx} \ast \dots \ast f_{\vx}}_{n \text{ times}})(h^{-1}(n \cdot \hat{\vb})) \\
\end{align}
In other words, an estimate of parameters from $n$ I.I.D. samples is just the estimation methodology $h$ applied to the assumed density $f_x$ convolved with itself $n$ times. 

Therefore, the PDF of $\hat{\theta}$ is:
\begin{equation}
    f_{\hat{\theta}}(\hat{\vb}) = P(H(\mX) = \hat{\vb}) = (\underbrace{f_{\vx} \ast \dots \ast f_{\vx}}_{n \text{ times}})\left(h^{-1}(n \cdot \hat{\vb})\right)
\end{equation}

% The expected value of $\hat{\theta}$ is thus
% \begin{equation}
%     \EX[\mX]{b} = \int_{b} b \cdot \left( f_{\vx} \ast \dots \ast f_{\vx} \right) \left(h^{-1} (n \cdot b ) \right) db
% \end{equation}
% \[
% \int_b b \cdot f_{\hat{\theta}}(b) db = \int_a a \cdot f_{\hat{\theta}}(a) da
% \]
